NELoRa-Bench: A Benchmark for Neural-enhanced LoRa Demodulation

Low-Power Wide-Area Networks (LPWANs) are an emerging Internet-of-Things (IoT) paradigm marked by low-power and long-distance communication. Among them, LoRa is widely deployed for its unique characteristics and open-source technology. By adopting the Chirp Spread Spectrum (CSS) modulation, LoRa enables low signal-to-noise ratio (SNR) communication. The standard LoRa demodulation method accumulates the chirp power of the whole chirp into an energy peak in the frequency domain. In this way, it can support communication even when SNR is lower than -15 dB. Beyond that, we proposed NELoRa, a neural-enhanced decoder that exploits multi-dimensional information to achieve significant SNR gain. This paper presents the dataset used to train/test NELoRa, which includes 27,329 LoRa symbols with spreading factors from 7 to 10, for further improvement of neural-enhanced LoRa demodulation. The dataset shows that NELoRa can achieve 1.84-2.35 dB SNR gain over the standard LoRa decoder. The dataset and codes can be found at https://github.com/daibiaoxuwu/NeLoRa_Dataset.

==> 2_related_work.tex <==
\section{Related Work}
\label{sec-related-work}

\cl{
\vspace{1mm}
\noindent
LoRa demodulation under low SNR is an essential topic in optimizing LPWAN performances, and in recent years, neural-based approaches have been used to optimize wireless communication systems~\citep{AIWirelessSensingSurvey_CSUR20}, such as the coding~\citep{29, 37, 46, 54} and decoding~\citep{49, 60, 33} mechanisms. However, For LoRa communication, only a few works have been proposed in this field. 
Specifically, ~\citet{deepLora} utilizes Bi-LSTM DNN to develop a land-cover aware path loss model and reduces the estimation error to less than 4 dB, which is 2$\times$ smaller than state-of-the-art~\citep{demetri_automated_2019} for link estimation.
~\citet{chan_deepsense_2019} further explores the deep learning augmented random access in the coexistence of LPWANs, even below the noise floor (e.g., -10dB).
Moreover, ~\citet{hessar_tinysdr_nodate} delivers FPGA-based hardware, which can boost the research on AI-augmented LoRa networks by supporting deep AI algorithms on board. 

Given the strong feature learning ability of DNN, we believe that AI augmentation brings a new direction to design a more efficient communication stack and sensing technique in LoRa networking. The previous works use relatively simple DNN models, and we believe that with the development of AI technology, more powerful models can be proposed with higher performance and lower computational cost.
However, the previous works only provide small datasets for open access, and to train a practical neural-based LoRa demodulation system, sufficient amounts of data with different parameters are crucial. In this paper, we provide a dataset with spreading factors 7 to 10, hoping to support future research on neural-based LoRa demodulation and provide a benchmark for the evaluation of LoRa demodulation methods.


